PowerFlowMultiNet: Multigraph Neural Networks for Unbalanced Three-Phase Distribution Systems

Efficiently solving unbalanced three-phase power flow in distribution grids is pivotal for grid analysis and simulation. There is a pressing need for scalable algorithms capable of handling large-scale unbalanced power grids that can provide accurate and fast solutions. To address this, deep learning techniques, especially Graph Neural Networks (GNNs), have emerged. However, existing literature primarily focuses on balanced networks, leaving a critical gap in supporting unbalanced three-phase power grids. This letter introduces PowerFlowMultiNet, a novel multigraph GNN framework explicitly designed for unbalanced three-phase power grids. The proposed approach models each phase separately in a multigraph representation, effectively capturing the inherent asymmetry in unbalanced grids. A graph embedding mechanism utilizing message passing is introduced to capture spatial dependencies within the power system network. PowerFlowMultiNet outperforms traditional methods and other deep learning approaches in terms of accuracy and computational speed. Rigorous testing reveals significantly lower error rates and a notable hundredfold increase in computational speed for large power networks compared to model-based methods.

==> pages/4.1-results2.tex <==
\begin{table*}[!hb]
\centering
\small
\caption{Results of PowerFlowMultiNet, GNN, and FCNN with real loads and perturbation of $\pm 10\%$ and $\pm 50\%$.} 
\label{results_uniform}
\resizebox{0.85\textwidth}{!}{
\begin{threeparttable}
    
    \small
\begin{tabular*}{1.2\linewidth}{ l l l | l l l l || l l }
    \toprule

Load       & Case    & Approach & $P_{MEAN}$\tiny{($STD$)}              & $Q_{MEAN}$\tiny{($STD$)}                      & $\phi_{MEAN}$\tiny{($STD$)}          & $V_{MEAN}$\tiny{($STD$)}   & Time$_{MEAN}$\tiny{($STD$)} & Time(Solver)$_{MEAN}$\tiny{($STD$)}           \\\midrule
$\pm 10\%$ & 13-Bus  & OURS     & \cellcolor[gray]{0.9} $2.47e^{-5}$\tiny{($2.35e^{-5}$)}   & $\cellcolor[gray]{0.9}2.61e^{-5}$\tiny{($2.11e^{-5}$)}           & $\cellcolor[gray]{0.9}5.72e^{-6}$\tiny{($2.4e^{-6}$)}  & $6.42e^{-6}$\tiny{($2.02e^{-6}$)} & $8.26e^{-6}$\tiny{($6.36e^{-7}$)}& $1.3e^{-4}$\tiny{($1.6e^{-4}$)}\\
           &         & GNN      & $4.35e^{-5}$\tiny{($4e^{-5}$)}      & $6.42e^{-5}$\tiny{($6.62e^{-5}$)}           & $1.15e^{-5}$\tiny{($6.26e^{-6}$)} & $\cellcolor[gray]{0.9}4.62e^{-6}$\tiny{($3.09e^{-6}$)}  & $1.05e^{-5}$\tiny{($1.2e^{-6}$)} & $\vert$\\
           &         & FCNN     & $2.23e^{-4}$\tiny{($2.24e^{-4}$)}   & $2.34e^{-4}$\tiny{($2.37e^{-4}$)}           & $7.43e^{-6}$\tiny{($4.91e^{64}$)} & $8.62e^{-6}$\tiny{($5.93e^{-6}$)} & $4.27e^{-6}$\tiny{($2.35e^{-7}$)} & $\vert$\\
           \cline{2-9}
           & 123-Bus & OURS     & \cellcolor[gray]{0.9}$1.26e^{-5}$\tiny{($1.5e^{-5}$)}    & \cellcolor[gray]{0.9}$1.09e^{-5}$\tiny{($1.08e^{-5}$)}           & \cellcolor[gray]{0.9}$2.02e^{-6}$\tiny{($2.55e^{-6}$)} & $1.18e^{-6}$\tiny{($6.2e^{-7}$)}   & $3.4e^{-5}$\tiny{($8.6e^{-6}$)}& $4.5e^{-4}$\tiny{($1.9e^{-4}$)}\\
           &         & GNN      & $2.41e^{-5}$\tiny{($2.24e^{-5}$)}   & $1.18e^{-5}$\tiny{($1.65e^{-5}$)}           & $3.69e^{-6}$\tiny{($1.99e^{-6}$)} & $\cellcolor[gray]{0.9} 9.92e^{-7}$\tiny{($6.11e^{-7}$)}  & $2.94e^{-5}$\tiny{($6.79e^{-6}$)} & $\vert$\\
           &         & FCNN     & $4.04e^{-5}$\tiny{($3.49e^{-5}$)}   & $2.88e^{-5}$\tiny{($2.52e^{-5}$)}           & $1.16e^{-5}$\tiny{($9.03e^{-6}$)} & $1.65e^{-6}$\tiny{($9.36e^{-7}$)}  & $2.11e^{-5}$\tiny{($4.04e^{-5}$)} & $\vert$\\
           \cline{2-9}
           & 906-Bus & OURS     & \cellcolor[gray]{0.9}$9.39e^{-8}$\tiny{($1.06e^{-7}$)}  & \cellcolor[gray]{0.9}$1.29e^{-7}$\tiny{($6.18e^{-8}$)}          & \cellcolor[gray]{0.9}$5.03e^{-6}$\tiny{($2.93e^{-6}$)} & \cellcolor[gray]{0.9}$4.31e^{-6}$\tiny{($2.39e^{-6}$)}  & $8.46e^{-5}$\tiny{($1.36e^{-5}$)}& $2.43e^{-3}$\tiny{($7.2e^{-4}$)}\\
           &         & GNN      & $4.57e^{-7}$\tiny{($4.37e^{-7}$)}  & $4.03e^{-7}$\tiny{($4.32e^{-7}$)}          & $2.28e^{-5}$\tiny{($4.20e^{-5}$)} & $8.45e^{-6}$\tiny{($6.64e^{-6}$)}  & $9.75e^{-6}$\tiny{($3.74e^{-7}$)} & $\vert$\\
           &         & FCNN     & $4.40e^{-7}$\tiny{($4.36e^{-7}$)} & $3.55e^{-7}$\tiny{($3.78e^{-7}$)} & $1.67e^{-5}$\tiny{($1.31e^{-6}$)} & $8.35e^{-6}$\tiny{($6.63e^{-6}$)} & $1.06e^{-6}$\tiny{($1.27e^{-7}$)} & $\vert$\\ \midrule
$\pm 50\%$ & 13-Bus  & OURS     & \cellcolor[gray]{0.9}$2.02e^{-4}$\tiny{($1.93e^{-4}$)}   & \cellcolor[gray]{0.9}$3.07e^{-4}$\tiny{($2.66e^{-4}$)}           & \cellcolor[gray]{0.9}$1.56e^{-5}$\tiny{($1.4e^{-5}$)}  & \cellcolor[gray]{0.9}$1.42e^{-5}$\tiny{($6.93e^{-6}$)}  & $1.01e^{-5}$\tiny{($6.49e^{-7}$)}& $1.9e^{-4}$\tiny{($1.7e^{-4}$)}\\
           &         & GNN      & $6.97e^{-4}$\tiny{($7.4e^{-4}$)}    & $5.91e^{-4}$\tiny{($6.13e^{-4}$)}           & $2.58e^{-5}$\tiny{($1.28e^{-5}$)} & $4.75e^{-5}$\tiny{($2.83e^{-5}$)}  & $1.06e^{-5}$\tiny{($1.29e^{-6}$)} & $\vert$\\
           &         & FCNN     & $2.27e^{-3}$\tiny{($2.56e^{-3}$)}   & $3.16e^{-3}$\tiny{($3.7e^{-3}$)}            & $1.02e^{-4}$\tiny{($6.03e^{-5}$)} & $1.16e^{-4}$\tiny{($7.16e^{-5}$)}  & $7.25e^{-6}$\tiny{($6.56e^{-6}$)} & $\vert$\\
           \cline{2-9}
           & 123-Bus & OURS     & \cellcolor[gray]{0.9}$6.28e^{-5}$\tiny{($5.7e^{-5}$)}    & \cellcolor[gray]{0.9}$4.68e^{-5}$\tiny{($3.76e^{-5}$)}            & \cellcolor[gray]{0.9}$1.07e^{-5}$\tiny{($8.94e^{-6}$)}  & \cellcolor[gray]{0.9}$5.27e^{-6}$\tiny{($2.73e^{-6}$)}  & $2.28e^{-5}$\tiny{($3.36e^{-7}$)}& $7.3e^{-4}$\tiny{($3.7e^{-4}$)}\\
           &         & GNN      & $3.75e^{-4}$\tiny{($3.63e^{-4}$)}   & $2.92e^{-4}$\tiny{($2.81e^{-4}$)}           & $1.44e^{-5}$\tiny{($8.62e^{-6}$)} & $1.61e^{-5}$\tiny{($8.84e^{-6}$)}  & $2.11e^{-5}$\tiny{($2.87e^{-7}$)} & $\vert$\\
           &         & FCNN     & $6.31e^{-4}$\tiny{($5.91e^{-4}$)}   & $2.92e^{-4}$\tiny{($5.03e^{-4}$)}           & $1.88e^{-5}$\tiny{($1.09e^{-5}$)} & $1.84e^{-5}$\tiny{($1.31e^{-5}$)} &  $7.76e^{-6}$\tiny{($2.26e^{-6}$)} & $\vert$\\
           \cline{2-9}
           & 906-Bus & OURS     & \cellcolor[gray]{0.9}$6.28e^{-7}$\tiny{($1.19e^{-7}$)}  & \cellcolor[gray]{0.9}$6.16e^{-8}$\tiny{($6.46e^{-8}$)}          & \cellcolor[gray]{0.9}$1.52e^{-5}$\tiny{($1.08e^{-5}$)} & \cellcolor[gray]{0.9}$2.2e^{-5}$\tiny{($1.47e^{-5}$)}  &  $6.68e^{-5}$\tiny{($2.11e^{-7}$)}& $2.53e^{-3}$\tiny{($6.1e^{-4}$)}\\
           &         & GNN      & $9.01e^{-6}$\tiny{($8.39e^{-6}$)}  & $7.43e^{-6}$\tiny{($7.5e^{-6}$)}          & $5.7e^{-5}$\tiny{($4.03e^{-5}$)} & $1.98e^{-4}$\tiny{($1.47e^{-4}$)}  & $9.51e^{-6}$\tiny{($1.55e^{-17}$)} & $\vert$\\
           &         & FCNN     & $1.07e^{-5}$\tiny{($1.03e^{-5}$)} & $8.42e^{-6}$\tiny{($8.07e^{-6}$)} & $4.15e^{-5}$\tiny{($3e^{-5}$)} & $2.03e^{-4}$\tiny{($1.51e^{-4}$)} & $8.90e^{-7}$\tiny{($9.04e^{-8}$)} & $\vert$\\ \midrule
Timeseries & 13-Bus  & OURS     & \cellcolor[gray]{0.9}$5.24e^{-4}$\tiny{($7.87e^{-4}$)}   & \cellcolor[gray]{0.9}$4.21e^{-4}$\tiny{($4.76e^{-4}$)}           & \cellcolor[gray]{0.9}$4.07e^{-5}$\tiny{($2.89e^{-5}$)} & \cellcolor[gray]{0.9}$2.66e^{-5}$\tiny{($2.28e^{-5}$)}  & $1.14e^{-5}$\tiny{($9.67e^{-7}$)}& $1.6e^{-4}$\tiny{($1e^{-4}$)}\\
           &         & GNN      & $1.19e^{-3}$\tiny{($1.53e^{-3}$)}   & $9.45e^{-3}$\tiny{($1.3e^{-3}$)}            & $4.47e^{-5}$\tiny{($3.51e^{-5}$)} & $6.95e^{-5}$\tiny{($6.78e^{-5}$)}  & $1.08e^{-5}$\tiny{($1.25e^{-6}$)} & $\vert$\\
           &         & FCNN     & $3.76e^{-3}$\tiny{($7.2e^{-3}$)}    & $4.32e^{-3}$\tiny{($8.21e^{-3}$)}           & $1.8e^{-4}$\tiny{($1.24e^{-4}$)}  & $1.71e^{-4}$\tiny{($1.84e^{-4}$)}  & $5.2e^{-5}$\tiny{($6.79e^{-5}$)} & $\vert$\\
           \cline{2-9}
           & 123-Bus & OURS     & \cellcolor[gray]{0.9}$1.09e^{-3}$\tiny{($1.16e^{-3}$)}   & \cellcolor[gray]{0.9}$8.44e^{-4}$\tiny{($8.4e^{-4}$)}            & \cellcolor[gray]{0.9}$5.22e^{-5}$\tiny{($2.65e^{-5}$)} & \cellcolor[gray]{0.9}$4.64e^{-5}$\tiny{($4.06e^{-5}$)}  & $2.76e^{-5}$\tiny{($3.51e^{-7}$)}& $1.03e^{-3}$\tiny{($5.6e^{-4}$)}\\
           &         & GNN      & $1.71e^{-3}$\tiny{($2.10e^{-3}$)}   & $1.56e^{-3}$\tiny{($2.44e^{-3}$)}           & $6.33e^{-5}$\tiny{($4.59e^{-5}$)} & $5.72e^{-5}$\tiny{($6.48e^{-5}$)}  & $2.12e^{-5}$\tiny{($3.51e^{-7}$)} &$\vert$\\
           &         & FCNN     & $3.68e^{-3}$\tiny{($5.82e^{-3}$)}   & $3.76e^{-3}$\tiny{($6.57e^{-3}$)}           & $8.21e^{-5}$\tiny{($5.94e^{-5}$)} & $8.42e^{-5}$\tiny{($1.15e^{-4}$)}  & $7.82e^{-6}$\tiny{($2.26e^{-6}$)} &$\vert$\\
           \cline{2-9}
           & 906-Bus & OURS     & \cellcolor[gray]{0.9}$2.15e^{-5}$\tiny{($2.25e^{-5}$)}  & \cellcolor[gray]{0.9}$1.15e^{-5}$\tiny{($1.2e^{-5}$)}           & \cellcolor[gray]{0.9}$4.58e^{-5}$\tiny{($2.05e^{-5}$)} & \cellcolor[gray]{0.9}$1.83e^{-4}$\tiny{($1.43e^{-4}$)}  & $6.66e^{-5}$\tiny{($2.37e^{-7}$)}& $2.46e^{-3}$\tiny{($5.6e^{-4}$)}\\
           &         & GNN      & $1.18e^{-4}$\tiny{($1.04e^{-4}$)}  & $7.7e^{-5}$\tiny{($7.83e^{-5}$)}          & $2.02e^{-4}$\tiny{($1.75e^{-4}$)} & $1.21e^{-3}$\tiny{($9.24e^{-4}$)}  & $9.48e^{-6}$\tiny{($1.4e^{-7}$)} &$\vert$\\
           &         & FCNN     & $4.2e^{-4}$\tiny{($4.05e^{-4}$)}  & $2.54e^{-4}$\tiny{($2.65e^{-4}$)}          & $2.11e^{-3}$\tiny{($2.7e^{-3}$)} & $2.32e^{-3}$\tiny{($1.56e^{-3}$)}  & $9.39e^{-7}$\tiny{($8.45e^{-8}$)} &$\vert$
\\             

\bottomrule
\end{tabular*}
\vspace{-1em}
\end{threeparttable}
}
\end{table*}

==> pages/6-bio.tex <==
\section{Biography Section}
If you have an EPS/PDF photo (graphicx package needed), extra braces are
 needed around the contents of the optional argument to biography to prevent
 the LaTeX parser from getting confused when it sees the complicated
 $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 simpler here.)
 
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}
